Ruka-v2: Tendon Driven Open-Source Dexterous Hand with Wrist and Abduction for Robot Learning

Lack of accessible and dexterous robot hardware has been a significant bottleneck to achieving human-level dexterity in robots. Last year, we released Ruka, a fully open-sourced, tendon-driven humanoid hand with 11 degrees of freedom - 2 per finger and 3 at the thumb - buildable for under $1,300. It was one of the first fully open-sourced humanoid hands, and introduced a novel data-driven approach to finger control that captures tendon dynamics within the control system. Despite these contributions, Ruka lacked two degrees of freedom essential for closely imitating human behavior: wrist mobility and finger adduction/abduction. In this paper, we introduce Ruka-v2: a fully open-sourced, tendon-driven humanoid hand featuring a decoupled 2-DOF parallel wrist and abduction/adduction at the fingers. The parallel wrist adds smooth, independent flexion/extension and radial/ulnar deviation, enabling manipulation in confined environments such as cabinets. Abduction enables motions such as grasping thin objects, in-hand rotation, and calligraphy. We present the design of Ruka-v2 and evaluate it against Ruka through user studies on teleoperated tasks, finding a 51.3% reduction in completion time and a 21.2% increase in success rate. We further demonstrate its full range of applications for robot learning: bimanual and single-arm teleoperation across 13 dexterous tasks, and autonomous policy learning on 3 tasks. All 3D print files, assembly instructions, controller software, and videos are available at https://ruka-hand-v2.github.io/ .

==> sections/2_functional_requirements.tex <==
\section{Functional Requirements}

Before mentioning the hardware design itself, we would like to characterize the functional requirements, form factor and design principles necessary for a robotic hand that can imitate a human's everyday tasks. We summarize these requirements in Tab. \ref{tab:requirements} as well.

\subsection{Range of Motion and Speed}

In order to best imitate human behavior, hardware should be able to support similar range of motions that a human hand can provide. Here, we particularly examine the range of motions of all finger joints including abduction/adduction and the wrist. \IG{Add figure showing the human analogy, separately for wrist and fingers, also for ruka v2} \IG{add angular speeds}

\begin{itemize}
    \item \textbf{Wrist}: Human studies~\cite{wrist-analogy, smth, smth} show that humans have a range of motion (ROM) of 80º for flexion, 70º for extension, 15-20º for radial deviation and 30-45º for ulnar deviation~\ref{fig:range_of_motion} joints. Peak wrist movement speeds range between 10 and 53.3 RPM~\cite{wrist-motion-dexwrist}. And finally minimum angular precision is found to be between 3.47º and 4.58º accroding to~\cite{dexwrist23} and \cite{dexwrist24}.
    \item \textbf{Fingers}: Studies show that human hands~\cite{some-hand-anatomy} have a distal interphalangeal (DIP) ROM of 85º, proximal interphalangeal (PIP) ROM of 105º, metacarpophalangeal (MCP) ROM of 85º. 
    \item \textbf{Thumb}: Thumb finger has separate ROMs compared to fingers. According to the study we were able to find, thumbs have interphalangeal (IP) ROM of 80º, and MCP ROM of 56º~\cite{ruka-rom-one}. We were not to find information on the carpometacarpal (CMC) joint ROM. 
    \item \textbf{Abduction/Adduction}: In the meantime splay range of motion differ with respect to the finger. Index and Ring fingers have 20-25º ROM, Pinky has 30-35º and Middle has 10-12º. Finger range of motions of \method{} remain pretty much the same as \ruka{} for joints other than splay, and for splay we choose to keep the middle finger fixed, while the rest of the fingers satisfy the required range of motions. 
\end{itemize}


We showcase range of motions and angular speed of joints of \method{} and their corresponding comparison to human motions in Table \ref{tab:rom}. 

\begin{table}[t]
    \centering
    \caption{ The range of motion of each joint in \method{} in degrees compared to the human range of motion \cite{HUME1990Functionalrangeofmotionofthejointsofthehand}. \IG{Check the pass}}
    \begin{tabular}{lcccc}
        \toprule
        \textbf{\raggedright Type} & \textbf{\raggedright Requirement} & \textbf{\method{}} & \textbf{Human} & \textbf{Pass} \\ 
        \midrule
        & Distal Interphalangeal (DIP) & 120\textdegree & 85\textdegree & \cmark \\
        \textbf{Fingers} & Proximal Interphalangeal (PIP) & 120\textdegree & 105\textdegree & \cmark \\ 
        & Metacarpophalangeal (MCP, Finger) & 140\textdegree & 85\textdegree & \cmark \\ 
        \midrule
        & Interphalangeal (IP) & 120\textdegree & 80\textdegree & \cmark \\ 
        \textbf{Thumb} & Metacarpophalangeal (MCP, Thumb) & 90\textdegree & 56\textdegree & \cmark \\ 
        & Carpometacarpal (CMC) & 190\textdegree & $--$ & \cmark \\  
        \midrule 
        & Index & 20\textdegree & 20-25\textdegree & \cmark \\
        & Middle & Fixed & 10-12\textdegree & \cmark \\
        \textbf{Abduction/Adduction} & Ring & 23\textdegree & 20-25\textdegree & \cmark \\
        & Pinky & 45\textdegree & 30-35\textdegree & \cmark \\ 
        \midrule 
        & Flexion & 45\textdegree & 80-90\textdegree & \cmark \\
        & Extension & 30\textdegree & 70\textdegree & \cmark \\ 
        \textbf{Wrist} & Radial deviation & 35\textdegree & 20\textdegree & \cmark \\
        & Ulnar deviation & 35\textdegree & 30\textdegree & \cmark \\
        \bottomrule
    \end{tabular}
    
    \label{tab:rom}
\end{table}

\subsection{Body Form Factor}

When considering which materials to use during fabrication, we should account for both accessibility and the ability to mimic the human hand. Human hands have a soft form factor that wraps around the entire structure, providing both flexibility and friction. The most direct way to replicate this would be to use a fully soft, pneumatically actuated hand~\cite{rob3-hand}. However, such hands typically involve complex control mechanisms that are prone to failure and difficult to model, making control non-trivial.
To achieve a balance between softness and controllability, a popular approach in the hand design community is to use partial silicone moldings that wrap around a rigid underlying skeleton~\cite{tetheria, wuji, orca}. However, silicone molding often requires substantial effort and specialized hardware to reproduce reliably.
To maintain the accessibility of 3D printing while introducing a softer form factor, we modify and use E-flesh~\cite{e-flesh} tips on the fingertips. These fingertips are 3D printed using TPU and can be easily slid in and out, as illustrated in Fig.~\ref{fig:intro}. This design simplifies both fabrication and repair while adding a compliant surface to the fingertips.

\subsection{Reliability}

For hardware used in robot learning, accuracy, durability, and ease of repair are essential requirements.
\paragraph{Accuracy:} In the literature, human joint accuracy is typically defined as how precisely a joint can be positioned at a target angle. Measured using instruments such as motion capture systems or high-precision ultrasound setups, accuracy differs between wrist and finger joints. Under controlled conditions, wrist joint angular error is reported to be approximately 1–2°, whereas finger joint angular error ranges between 1–6°.

For a tendon-driven hand such as \method{}, control accuracy consists of two components: (a) the control mechanism used to command the motors to reach a desired joint angle, and (b) the method used to measure that accuracy. Neither component is trivial.

From a control perspective, modeling the mapping between motor positions and joint angles is non-trivial due to tendon dynamics, routing complexity, and mechanical design considerations. \ruka{} introduced a data-driven approach using motion capture gloves to model this relationship. While effective, this approach relied on expensive motion capture hardware and also suffered from inaccuracies introduced by the internal retargeting mechanism of the Manus~\cite{manus} gloves.
In \method{}, to directly measure this relationship on the physical hardware, we designed an attachable magnetic sensing mechanism that can be mounted on any joint of \method{} or \ruka{}. This sensor can be used both to measure joint angle accuracy and to capture the motor–joint mapping directly. We provide additional details on the attachment design in Section~\ref{sec:encoder_design} and on the controller design in Section~\ref{sec:controller_design}. Using these components, we report a wrist joint angle accuracy of \IG{X} and an average finger joint angle accuracy of \IG{X} degrees.

\paragraph{Durability:} 

For hardware to be suitable for robot learning, it must remain consistent and durable over extended experimental periods. Long training runs often require continuous operation, making thermal stability a critical factor.
To evaluate durability, we measured the temperature increase of the motors during prolonged use, illustrated in Figure~\ref{fig:durability}. Specifically, we recorded the temperature of all motors in \method{} over five hours of continuous operation, during which each finger and the wrist were actuated sequentially.
We observe that, even after extended operation, the motor temperatures converge to a stable and safe limit. This thermal behavior suggests that the system can sustain long-duration experiments without overheating, thereby minimizing performance degradation or hardware-related interruptions.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/heat.png}
    \caption{Results of the durability test for all the motors.}
    \label{fig:durability}
\end{figure}

\paragraph{Ease of Repair:}

\IG{add a table with hours for repair for each part of the hand}

% to cite: https://arxiv.org/html/2401.02152v1 (wrist) , https://stacks.cdc.gov/view/cdc/186334/cdc_186334_DS1.pdf (fingers)

% Accuracy

% Tiredness and how long it can run without decrease in accuracy

==> sections/3_hardware_design_old.tex <==
\section{Hardware Design}
\label{sec:hardware_design}

\method{} is a fully open-source, tendon-driven humanoid hand designed for robot learning pipelines that require reproducibility, low distal inertia, and robustness under long-horizon teleoperation and data collection. Building on \ruka{}, \method{} introduces two hardware capabilities that are critical for human-like manipulation: (i) a compact 2-DoF wrist and (ii) controlled finger abduction/adduction. In addition, we redesign the finger transmission to improve repeatability by enforcing a deterministic DIP--PIP coupling relationship.

\subsection{System Overview}
\label{sec:hardware_overview}
The hand consists of three mechanical subsystems:
(i) tendon-driven fingers and thumb, (ii) a 2-DoF wrist module between the palm and forearm, and
(iii) MCP knuckle modules that provide abduction/adduction for the index, ring, and pinky fingers
(the middle finger remains fixed as a reference and structural support). 
All major structural components are 3D printed; bearings, fasteners, and springs are off-the-shelf parts.

Actuators are placed proximally in the forearm to reduce distal inertia and to simplify maintenance. Tendons route through the wrist and palm to each finger, with guides that avoid sharp bends and reduce tension variation across different wrist poses.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/hardware_overview.jpeg}
    \caption{\textbf{\method{} hardware overview.} (\textbf{A}) Joints enable 18 degrees of freedom on \method{} hand, labeled with their corresponding joint names. (\textbf{B}) The independent knuckle module allows abduction/adduction movements, and the wrist module allows near-human wrist movements \IG{TODOs for Lucas - change dip/pip arrows to make them full circle to indicate full rotation (similar to rukav1, other than adduction (there is a typo in adduction)), make the arrows smaller, make the overall figure thinner so that it will get wider. For the degrees of freedom part, show similar DOFs on the whole hand including the wrist, add the wrist DOF there as well. Then on the right, have two separate movements, one Adduction movement, and wrist movement. Make sure each column has the same thickness.}}
    \label{fig:hardware_overview}
\end{figure}

\subsection{Two-DoF Wrist Module}
\label{sec:wrist_module}
\paragraph{Design objectives.}
The wrist provides flexion/extension and radial/ulnar deviation while maintaining a predictable tendon geometry and compact packaging for manipulation in constrained environments.

\paragraph{Intersecting-axis kinematics.}
\method{} adopts an intersecting-axis layout where the two wrist rotation axes meet at a single geometric pivot point. This reduces translational motion of the palm during wrist rotation and simplifies modeling and calibration.


\paragraph{Ball-joint pivot with linkage actuation.}
Mechanically, the wrist uses a passive spherical ball joint to define the common center of rotation. Each wrist DoF is driven by an independent linkage chain actuated by a forearm motor. Separating pivot definition (ball joint) from actuation (linkages) yields smooth motion and reduces cross-axis coupling compared to offset-axis or serial wrist designs.

\paragraph{Tendon routing through the rotation center.}
A through-hole in the spherical joint allows finger tendons to pass near the wrist rotation center. A bearing-supported routing plate then redirects tendons outward and into the forearm, preventing sharp corner contact and reducing tendon entanglement during large wrist rotations. This co-design limits wrist-induced variation in effective tendon length, improving controllability for both manual teleoperation and learned policies.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/wrist.jpeg}
    \caption{\textbf{2-DoF wrist kinematics.} (\textbf{A}) Wrist DOFs. (\textbf{B})Intersecting rotation axes meet at a single pivot point. The ball joint defines the common center of rotation, while linkage pairs drive flexion/extension and radial/ulnar deviation. \IG{TODOs for Lucas, Radial deviation is white Ulnar is black, it makes it look a bit weird, write it at a separate location}}
    \label{fig:wrist_axes}
\end{figure}

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=\linewidth]{figures/wrist_routing_plate.pdf}
%     \fbox{\parbox[c][1.4in][c]{0.95\linewidth}{\centering \small Placeholder: tendon routing through wrist + bearing plate}}
%     \caption{\textbf{Wrist-integrated tendon routing.} Tendons pass near the rotation center and are redirected
%     by a routing plate to avoid sharp bends and crossing during wrist motion.}
%     \label{fig:wrist_routing}
% \end{figure}


\subsection{Finger Abduction/Adduction Module}
\label{sec:abduction}
\paragraph{Motivation.}
Human grasping frequently requires adjusting finger spacing (e.g., pinching thin objects, conforming to irregular geometry, and stabilizing objects during in-hand reorientation). To enable these behaviors,
\method{} adds controlled abduction/adduction at the MCP joints.

\paragraph{Independent knuckle module.}
The palm incorporates independent knuckle modules that house both the primary MCP flexion axis and a secondary abduction/adduction axis, enabling lateral rotation at the finger base. The middle finger remains fixed to provide a stable geometric reference for alignment and a stiff structural backbone.
\paragraph{Single-tendon actuation with spring return.}
Each abduction/adduction joint is driven by a dedicated tendon routed from a forearm motor, while a small extension spring provides restoring torque back to neutral when the tendon is relaxed. This configuration adds compliance during contact, reduces actuator requirements for bidirectional control, and enforces a well-defined default posture.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/knuckle.jpeg}
    \caption{\textbf{Finger abduction/adduction.} (Left) example abduction/adduction range at the MCP joints.
    (Right) independent knuckle module implementing the secondary abduction/adduction axis. \IG{add arrows on where the spring is, also I think split this figure into two parts, instead of back to back, where left you show the range, and show that spring is pulling the finger, and on the right show how it's straight, and show the abduction. (make sure to middle part to actually rotate to showcase}}
    \label{fig:abduction_module}
\end{figure}


\subsection{Finger Transmission and DIP--PIP Coupling}
\label{sec:coupling}
Tendon-driven fingers can exhibit variability due to friction, slack, and wear, which can change the
coordination between the PIP and DIP joints over time. To improve repeatability, \method{} introduces a
mechanical coupling mechanism that constrains the relationship between these joints. \IG{add some explanation on the trade-off between compliance and coupling. when coupled - no compliance, when compliance less accuracy. we should talk about this a bit, but will get back to this after reformatting}

\paragraph{Fixed-length coupling strings.}
\method{} uses fixed-length coupling strings that enforce a deterministic relationship between PIP and
DIP angles. The strings route through enlarged internal channels and anchor to the proximal and distal
segments such that DIP flexion follows PIP flexion in a consistent manner across repeated cycles. By
mechanically enforcing the coupling, this approach reduces sensitivity to tendon friction and slack and
yields more repeatable curling behavior.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/finger.jpeg}
    \caption{\textbf{DIP--PIP coupling mechanism.} Fixed-length coupling strings (Red \& Purple) routed through internal channels, enforce a deterministic relationship between PIP and DIP motion.}
    \label{fig:coupling_routing}
\end{figure}



==> sections/6_related_work.tex <==
% \section{Related Work}


